COOLer: Class-Incremental Learning for Appearance-Based Multiple Object Tracking

Continual learning allows a model to learn multiple tasks sequentially while retaining the old knowledge without the training data of the preceding tasks. This paper extends the scope of continual learning research to class-incremental learning for multiple object tracking (MOT), which is desirable to accommodate the continuously evolving needs of autonomous systems. Previous solutions for continual learning of object detectors do not address the data association stage of appearance-based trackers, leading to catastrophic forgetting of previous classes' re-identification features. We introduce COOLer, a COntrastive- and cOntinual-Learning-based tracker, which incrementally learns to track new categories while preserving past knowledge by training on a combination of currently available ground truth labels and pseudo-labels generated by the past tracker. To further exacerbate the disentanglement of instance representations, we introduce a novel contrastive class-incremental instance representation learning technique. Finally, we propose a practical evaluation protocol for continual learning for MOT and conduct experiments on the BDD100K and SHIFT datasets. Experimental results demonstrate that COOLer continually learns while effectively addressing catastrophic forgetting of both tracking and detection. The code is available at https://github.com/BoSmallEar/COOLer.

==> main_tables/ablation_ct_loss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\scriptsize
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.6}
\begin{tabular}{@{}lcccccc@{}}
\toprule
 
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Setting}\\ Stage (+New Classes)\end{tabular}}                                        & \multicolumn{2}{c}{Components} & \multicolumn{4}{c}{All Classes}   \\\cmidrule(l){2-3} \cmidrule(l){4-7}                                                                               & PL & CT Loss                      & mMOTA          & mHOTA          & mIDF1          & mAP            \\ \midrule  
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 1 \\ (+Pedestrian)\end{tabular}} & Det      & \xmark                         & 46.7     &     49.5          &  59.2             &      46.8          \\  
                                                                                            & Track      & \xmark                         & 54.1          & \textbf{52.6}          & \textbf{64.5} & 47.2  \\  
                                                                                            & Track      & OWOD~\cite{joseph2021towards} & 53.7 & 52.2 & 63.9          &    47.2       \\   
                                                                                            & Track      & Ours                          & \textbf{54.2} & \textbf{52.6} & 64.3          &  \textbf{47.4}         \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 2 \\ (+Truck)\end{tabular}}      & Det      & \xmark                    & 34.9 & 47.1 &55.6 &   42.5          \\  
                                                                                            & Track     & \xmark                     & \textbf{43.4} & 49.1          & 59.5          & \textbf{42.8}        \\  
                                                                                            & Track      & OWOD~\cite{joseph2021towards}  & 41.9          & 48.7 & 58.9 &   \textbf{42.8}  \\  
                                                                                            & Track      & Ours                      & 42.8          & \textbf{49.2} & \textbf{59.6} &  42.6   \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 3 \\ (+Bus)\end{tabular}}        & Det      & \xmark                 & 14.1 &43.1 &49.1&  40.9        \\\ 
                                                                                            & Track      & \xmark                      & 32.8          & 47.6          & 56.9          &     \textbf{41.9}      \\  
                                                                                            & Track      & OWOD~\cite{joseph2021towards}  &  33.1 &  47.5 & 56.9 & \textbf{41.9}  \\  
                                                                                            & Track      & Ours                       & \textbf{34.0} & \textbf{47.9} & \textbf{57.3} & \textbf{41.9}  \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 4 \\ (+Bicycle)\end{tabular}}    & Det      & \xmark           & 3.6 & 37.6 & 42.4 &  34.3    \\  
                                                                                            & Track     & \xmark                  & 25.7          & 43.9          & 52.9          &  36.1  \\   
                                                                                            & Track   & OWOD~\cite{joseph2021towards} & 24.7 & 43.7 & 52.7 &  36.1          \\  
                                                                                            & Track   & Ours                   & \textbf{28.6} & \textbf{44.4} & \textbf{53.9} &   \textbf{36.5}       \\ \bottomrule  
\end{tabular}
\caption{\textbf{Ablation Study on Method Components.}  We ablate on the choice of pseudo-labels (PL) and contrastive (CT) loss for COOLer on Most$\rightarrow$Least setting on BDD100k. We compare training with our proposed  pseudo-labels generated by the tracker (Track) and the pseudo-labels generated by the detector (Det). We also compare our proposed contrastive loss (Ours) with the contrastive loss proposed in OWOD~\cite{joseph2021towards}.}
\label{tab:ab_ct_loss}
\end{table*}

==> main_tables/bdd_exp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[h!]
\centering
\scriptsize
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.6}
\begin{tabular}{@{}llcccc@{}}
\toprule \toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Setting}\\ Stage (+New Classes)\end{tabular}}                                              &       & \multicolumn{4}{c}{All Classes}                                                                                         \\ \cmidrule(l){3-6} 
&Method                                                                   & mMOTA          & mHOTA          & mIDF1          & mAP                    \\ \midrule \midrule

\textbf{M}$\rightarrow$\textbf{L}  Stage 0 (Car) &   &  67.6 & 62.1 & 73.3 & 58.7 \\
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 1 (+Pedestrian) \end{tabular}}     & Fine-tuning    & 15.6      & 21.8       &27.7           & 19.9                  \\ 
                                                                                                & Distillation &   46.4        &  51.7        & 63.0         & 47.1                      \\  
                                                                                                & Det PL      &   46.7       &  49.5        & 59.2          &  46.8                           \\  
                                                                                                & COOLer        & \textbf{54.2}  &  \textbf{52.6}& \textbf{64.3} & \textbf{47.4}  \\  
                                                                                               &  \cellcolor{lightgray}Oracle       & \cellcolor{lightgray}57.4 & \cellcolor{lightgray}53.6 & \cellcolor{lightgray}65.9 & \cellcolor{lightgray}48.3            \\\midrule 
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 2 (+Truck)\end{tabular}}          & Fine-tuning    &   -11.5        & 12.8         & 14.0           &  11.7           \\ 
                                                                                                & Distillation &     27.3     &   47.8     &    57.3       &  \textbf{42.8}                      \\  
                                                                                                & Det PL      &  34.9         & 47.1          &55.6           & 42.5              \\  
                                                                                                & COOLer      & \textbf{42.8}  & \textbf{49.2} &  \textbf{59.6}     & 42.6           \\ 
                                                                                                 & \cellcolor{lightgray}Oracle      & \cellcolor{lightgray}49.8 & \cellcolor{lightgray}50.8 &  \cellcolor{lightgray}62.1     & \cellcolor{lightgray}45.0           \\ \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 3  (+Bus)\end{tabular}}            & Fine-tuning           &  -24.0           & 9.2        & 9.3 &  9.9           \\  
                                                                                                & Distillation           &  -11.2         &   43.4         &  50.8          &  40.8                \\  
                                                                                                & Det PL       &  14.1         &    43.1     &     49.1       &   40.9         \\  
                                                                                                & COOLer        &  \textbf{34.0} &  \textbf{47.9} & \textbf{57.3}  & \textbf{41.9}     \\
                                                                                                & \cellcolor{lightgray}Oracle      & \cellcolor{lightgray}45.4  & \cellcolor{lightgray}50.1  &  \cellcolor{lightgray}60.9 &\cellcolor{lightgray}44.5       \\\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 4  (+Bicycle)\end{tabular}}        & Fine-tuning          &  -16.0           & 5.6          & 6.5         &4.6            \\ 
                                                                                                & Distillation          &    -19.4        &   40.1         &   47.1         &  35.1                               \\ 
                                                                                                & Det PL           &   3.6       &   37.6        &  42.4         &  34.3           \\  
                                                                                                & COOLer       & \textbf{28.6}   &   \textbf{44.4}&  \textbf{53.9} &  \textbf{36.5}           \\
                                                                                                   & \cellcolor{lightgray}Oracle       & \cellcolor{lightgray}41.3  & \cellcolor{lightgray}47.1  & \cellcolor{lightgray}58.0  & \cellcolor{lightgray}39.9       \\\midrule \midrule
 \textbf{G}$\rightarrow$\textbf{S}  Stage 0 (General)  & &   45.6  &  50.3 &  61.1&  44.6  \\
\midrule                                                                                                 
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{G}$\rightarrow$\textbf{S}\\ Stage 1 (+Specific)\end{tabular}} & Fine-tuning              &   -24.7      & 11.7         & 14.1          &  8.4               \\  
                                                                                                & Distillation          &    -32.9      &  35.4         &  42.4         & 29.5         \\  
                                                                                                & Det PL                &   6.0        &  34.9         & 41.5         &  27.9       \\  
                                                                                                & COOLer         & \textbf{28.6} &  \textbf{38.5}&  \textbf{48.2}&  \textbf{29.9}              \\ 
                                                                                                & \cellcolor{lightgray}Oracle         &  \cellcolor{lightgray}30.4 & \cellcolor{lightgray}38.9  &  \cellcolor{lightgray}49.0      &\cellcolor{lightgray}30.9    \\ \midrule \midrule
                                                                                               \textbf{V}$\rightarrow$\textbf{B}$\rightarrow$\textbf{H}  Stage 0 (Vehicle) & & 33.1    & 39.2  & 46.8   & 35.0   \\
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{V}$\rightarrow$\textbf{B}$\rightarrow$\textbf{H}\\ Stage 1 (+Bike)\end{tabular}}   & Fine-tuning            &   -27.5     &  9.7          & 11.2            &    7.3             \\ 
                                                                                                & Distillation          &  -30.5         & 34.1          &  39.6 & \textbf{29.1}              \\  
                                                                                                & Det PL               &      -3.3     &     31.3      &    37.0       &    26.7      \\  
                                                                                                & COOLer        & \textbf{24.4}  & \textbf{36.8} &   \textbf{44.8}        &    \textbf{29.1}             \\ 
                                                                                                & \cellcolor{lightgray}Oracle        & \cellcolor{lightgray}27.6 & \cellcolor{lightgray}38.5 & \cellcolor{lightgray}47.8    & \cellcolor{lightgray}30.8              \\ \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{V}$\rightarrow$\textbf{B}$\rightarrow$\textbf{H}\\ Stage 2 (+Human)\end{tabular}}  & Fine-tuning        &  7.4        & 10.0          & 13.1           &  8.2      \\  
                                                                                                & Distillation         &  14.8         &   35.8        & 43.9          &   27.9               \\  
                                                                                                & Det PL         & 15.5          &   34.6        &   41.5        &   27.4       \\  
                                                                                                & COOLer       & \textbf{27.1} &  \textbf{37.5}&  \textbf{46.8}&  \textbf{28.8}           \\ 
                                                                                                 &\cellcolor{lightgray}Oracle       & \cellcolor{lightgray}30.4 & \cellcolor{lightgray}38.9 &  \cellcolor{lightgray}49.0 & \cellcolor{lightgray}30.9       \\ \bottomrule \bottomrule 
\end{tabular}
\caption{ \footnotesize\textbf{Class-incremental Learning on \bdd.} We conduct experiments on Most$\rightarrow$Least, General$\rightarrow$Specific and Vehicle$\rightarrow$Bike$\rightarrow$Human settings.
We compare COOLer with the Fine-tuning, Distillation, Det PL baselines and the oracle tracker.  }
\label{tab:bdd_exp}
\end{table*}
% \tao{for this table and the next table: does it make sense to have the horizontal line disconnect between different ``xxx classes''? this could make the split of different classes more clear.}

==> main_tables/shift_exp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\scriptsize
\setlength\tabcolsep{3pt}
\renewcommand\arraystretch{0.6}
\begin{tabular}{@{}llcccc @{}}
\toprule \toprule
% \multicolumn{2}{l}{\multirow{2}{*}{SHIFT Experiments}}
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Setting}\\ Stage (+New Classes)\end{tabular}} & & \multicolumn{4}{c}{All Classes}                                                                                \\ \cmidrule(l){3-6} 
 & Method                                                                  & mMOTA          & mHOTA          & mIDF1          & mAP                       \\ \midrule \midrule

\textbf{M}$\rightarrow$\textbf{L}  Stage 0 (Pedestrian) &  & 53.7   &  46.1  &  54.4   &   43.0    \\
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 1 (+Car) \end{tabular}}     & Fine-tuning    &  25.8   &  28.5    &   30.9       &   25.3           \\ 
                                                                                                % & Distillation   &  49.2 &   49.3 &  56.2  &  43.5   & \textbf{51.2}  &  44.3  &  \textbf{53.3}  &  40.3  & 47.2  & 54.4  &  59.1 &  46.8         \\  
                                                                                                & Det PL      &  44.6        & 46.8         & 49.7         &  45.6                              \\  
                                                                                                & COOLer     & \textbf{50.9}  & \textbf{50.9}  & \textbf{57.0}  &  \textbf{45.7}            \\ 
                                                                                               &  \cellcolor{lightgray}Oracle       & \cellcolor{lightgray}53.7& \cellcolor{lightgray}51.8& \cellcolor{lightgray}58.7& \cellcolor{lightgray}46.2            \\\midrule 
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 2 (+Truck)\end{tabular}}          & Fine-tuning    &   11.7      &  18.0        &   19.6         &   15.5                 \\ 
                                                                                                % & Distillation &          &       &         &          &           &           &           &                 &          &        &           &                   \\  
                                                                                                & Det PL      &     34.6      &   44.7       &    45.9      &    \textbf{44.8 }            \\  
                                                                                                & COOLer      & \textbf{45.2}   &\textbf{ 51.5}   &\textbf{ 57.3} &  \textbf{44.8}       \\ 
                                                                                                 & \cellcolor{lightgray}Oracle      & \cellcolor{lightgray}52.6 & \cellcolor{lightgray}53.5 &  \cellcolor{lightgray}60.7    & \cellcolor{lightgray}46.0      \\ \midrule
% \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 3  (+Motorcycle)\end{tabular}}            & Fine-tuning           &   9.4     & 13.3       & 14.5 & 11.3        & 0.0           & 0.0           & 0.0           & 0.0           &    37.6      &   53.2                &  58.1          &   45.1       \\  
%                                                                                                 & Distillation           &           &           &           &            &           &            &          &          &        &             &           &           \\  
%                                                                                                 & Det PL       &     33.2      &   43.1     &   44.3       &  43.9     &   32.1     &  39.8     & 39.3         &  43.5          &   36.6       &   52.8        &   59.1        & 44.9  \\  
%                                                                                                 & COOLer        & 42.8   &  51.7   &  57.6 &  44.0 & 42.7  & 50.9 & 56.3   & 44.1  & 42.8 & 54.0  & 61.4  &  43.7    \\
%                                                                                                 & \cellcolor{lightgray}Oracle      & \cellcolor{lightgray} 52.1 & \cellcolor{lightgray} 53.7 &  \cellcolor{lightgray} 60.5  &\cellcolor{lightgray} 45.9   & \cellcolor{lightgray} 52.6 & \cellcolor{lightgray} 53.5& \cellcolor{lightgray} 60.7 & \cellcolor{lightgray} 46.0 & \cellcolor{lightgray} 50.4 & \cellcolor{lightgray} 54.2  &\cellcolor{lightgray} 59.9   & \cellcolor{lightgray} 45.4    \\\midrule \midrule
  \textbf{G}$\rightarrow$\textbf{S}  Stage 0 (General)  & &  50.8  & 53.1 & 60.0 & 46.0   \\ \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{G}$\rightarrow$\textbf{S}\\ Stage 1 (+Specific)\end{tabular}} & Fine-tuning          & 19.4          & 24.1          & 26.9          &    20.0               \\  
 % & Distillation  &   42.9        &   49.2       &   56.3      &    41.3        &      \textbf{50.4}     & 51.1     &    58.9     &     42.8     &   35.3      &  47.3       &   53.7     &     39.8    \\  
                                                                                               & Det PL   & 45.8          & 49.8          & 55.4          &    \textbf{43.2}        \\  
                                                                                               & COOLer      &  \textbf{46.0} & \textbf{50.8} & \textbf{57.0} &    42.7                \\ 
                                                                                                &\cellcolor{lightgray}Oracle   &  \cellcolor{lightgray}48.8       &  \cellcolor{lightgray}51.1        & \cellcolor{lightgray}57.5         &  \cellcolor{lightgray}43.8       \\  
                                                                                               \midrule \midrule
                                                                                                \textbf{V}$\rightarrow$\textbf{B}$\rightarrow$\textbf{H}  Stage 0 (Vehicle) & &   47.2  & 52.1  & 57.4   & 45.2  \\ \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{V}$\rightarrow$\textbf{B}$\rightarrow$\textbf{H}\\ Stage 1 (+Bike)\end{tabular}}   & Fine-tuning          & 16.1          & 20.4          & 22.4          &       16.6               \\  
 % & Distillation   &   42.9       &  49.5        &  55.9    &   40.7   &    \textbf{48.3}      &   \textbf{50.9}       &   57.2     &    43.1   &  34.7  &  47.5  &  54.0  &  37.0\\  
                                                                                               & Det PL            & 39.4          & 47.1          & 51.0          &   42.0             \\  
                                                                                               & COOLer    &  \textbf{44.5} & \textbf{51.3} & \textbf{57.5} &  \textbf{42.3}  
                                                                                               \\ 
                                                                                                &\cellcolor{lightgray}Oracle   &  \cellcolor{lightgray}47.8        & \cellcolor{lightgray}52.1         & \cellcolor{lightgray}58.0         & \cellcolor{lightgray}44.2      \\  \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{V}$\rightarrow$\textbf{B}$\rightarrow$\textbf{H}\\ Stage 2  (+Human)\end{tabular}}  & Fine-tuning            & 8.9           & 7.7           & 9.1           &          7.1          \\  
 % & Distillation   &          &          &           &         &           &          &           &          &   &   &   &  \\  
                                                                                               & Det PL            & 37.3          & 41.4          & 43.7          &     41.7              \\  
                                                                                               & COOLer    &\textbf{ 47.0} & \textbf{ 50.6} &  \textbf{57.5} & \textbf{42.2}     \\ 
                                                                                                &\cellcolor{lightgray}Oracle   &    \cellcolor{lightgray}48.8    &  \cellcolor{lightgray}51.1       &    \cellcolor{lightgray}57.5     &  \cellcolor{lightgray}43.8      \\  \bottomrule \bottomrule
\end{tabular}
\caption{\textbf{Class-incremental Learning on \shift.} We conduct experiments on Most$\rightarrow$Least, General$\rightarrow$Specific and Vehicle$\rightarrow$Bike$\rightarrow$Human settings.
We compare COOLer with the Fine-tuning and Det PL baselines and the oracle tracker.}
\label{tab:shift_exp}
\end{table*}

==> sections/0_abstract.tex <==
% \begin{abstract}
% Continual learning allows the model to learn multiple tasks sequentially and retain the old knowledge without the training data of the preceding tasks. This paper extends the scope of continual learning research by addressing continual learning for multi-object tracking (MOT), which is desirable as MOT datasets are expensive to collect. Previous methods have been proposed to alleviate forgetting of the object detector. However, they do not address catastrophic forgetting in object association, leading to poor tracking performance. We propose to use tracking pseudo labels which have both detection and association information for object of previous classes, so the previous knowledge can be preserved. Besides that, we introduce a novel contrastive loss that can better disentangle the latent representations of objects from different classes and reduce misclassifications and wrong associations, which further boosts the performance. To evaluate continual learning for MOT methods, we propose a practical evaluation protocol and conduct experiments on the BDD100k dataset and SHIFT dataset. The results demonstrate that our method can improve both the tracking and detection performance compared to continual learning for object detection methods. We hope our work can serve as a starting point for further research. 
% \end{abstract}

\begin{abstract}
%
% \mattia{Consider changing the title to `COOLer: Continual Contrastive Learning for Multiple Object Tracking'}
%
Continual learning allows a model to learn multiple tasks sequentially while retaining the old knowledge without the training data of the preceding tasks. 
%
This paper extends the scope of continual learning research by addressing class-incremental learning for \ac{mot}, which is desirable to accommodate the continuously evolving needs of practitioners.
%
Previous solutions for continual learning of object detectors do not address the data association stage of tracking-by-detection systems, leading to catastrophic forgetting of previous classes' re-identification features.
%
% Previous methods have been proposed to alleviate forgetting of the object detector. 
%
% However, they do not address catastrophic forgetting in object association, leading to poor tracking performance.
%
We introduce COOLer, a COntrastive- and cOntinual-Learning-based tracker, which preserves past knowledge by training on a combination of currently available ground truth labels and pseudo-labels generated by the past tracker. 
% \mattia{maybe switch continual and contrastive as in the proposed title and rephrase as `We introduce COOLer, a COntrastive- and cOntinual-Learning-based tracker which ...'}
%
% We propose to use tracking pseudo labels which have both detection and association information for object of previous classes, so the previous knowledge can be preserved.
%
To further exacerbate the disentanglement of latent class representations, we introduce a novel class-incremental contrastive loss that favors tracking by improving detection performance and reducing misclassifications.
% \mattia{...contrastive loss that favors tracking by improving detection performance and reducing misclassifications}.
%
% Besides that, we introduce a novel contrastive loss that can better disentangle the latent representations of objects from different classes and reduce misclassifications and wrong associations, which further boosts the performance. 
%
Finally, we propose a practical evaluation protocol for continual learning for MOT and conduct experiments on the \bdd and \shift dataset. 
%
% To evaluate continual learning for MOT methods, we propose a practical evaluation protocol and conduct experiments on the BDD100k dataset and SHIFT dataset. 
%
Experimental results demonstrate that COOLer effectively addresses catastrophic forgetting of both tracking and detection. 
% The results demonstrate that our method can improve both the tracking and detection performance compared to continual learning for object detection methods. 
%
% We hope our work can serve as a starting point for further research. 
\end{abstract}

==> sup_tables/ab_full_overall.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\scriptsize
\setlength\tabcolsep{1.9pt}
\renewcommand\arraystretch{0.9}
\begin{tabular}{@{}lccccc|ccc@{}}
\toprule
 
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Setting}\\ Stage (+New Classes)\end{tabular}}                                        & \multicolumn{2}{c}{Components}   & \multicolumn{3}{c}{Old Classes} & \multicolumn{3}{c}{New Classes} \\\cmidrule(l){2-3} \cmidrule(l){4-9}                                                                         & PL & CT Loss                      &  MOTA         & HOTA          & IDF1    &  MOTA         & HOTA          & IDF1                   \\ \midrule  
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 1 \\ (+Pedestrian)\end{tabular}} & Det      & \xmark                  &60.1&55.7&63.0&33.3&43.4&55.4  \\  
                                                                                            & Track      & \xmark                    &65.8&61.6&72.5&\textbf{42.5}&\textbf{43.7}&\textbf{56.6}\\  
                                                                                            & Track      & OWOD~\cite{joseph2021towards}    &65.4&61.3&72.1&42.0&43.1&55.6   \\   
                                                                                            & Track      & Ours                  &\textbf{66.0}&\textbf{61.8}&\textbf{72.8}&\textbf{42.5}&43.4&55.8 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 2 \\ (+Truck)\end{tabular}}      & Det      & \xmark            &60.8&56.5&66.3&6.4&42.9&49.3      \\  
                                                                                            & Track     & \xmark      &60.2&58.3&69.2&\textbf{29.5}&\textbf{44.3}&\textbf{52.7}    \\  
                                                                                            & Track      & OWOD~\cite{joseph2021towards}   &59.6&58.1&69.0&27.6&43.8&51.7\\  
                                                                                            & Track      & Ours            &\textbf{60.8}&\textbf{58.7}&\textbf{69.6}&26.7&43.9&52.1 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 3 \\ (+Bus)\end{tabular}}        & Det      & \xmark           &55.9&53.9&62.1&-53.2&40.0&42.8  \\\ 
                                                                                            & Track      & \xmark                   &55.4&56.5&67.1&10.2&45.8&52.8 \\  
                                                                                            & Track      & OWOD~\cite{joseph2021towards}  &54.7&56.3&66.8&\textbf{14.6}&\textbf{46.2}&\textbf{53.8}\\  
                                                                                            & Track      & Ours         &\textbf{56.8}&\textbf{57.1}&\textbf{67.8}&12.4&\textbf{46.2}&53.3 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{M}$\rightarrow$\textbf{L}\\ Stage 4 \\ (+Bicycle)\end{tabular}}    & Det     & \xmark   &41.2&43.2&46.2&-57.6&29.7&34.5 \\  
                                                                                            & Track     & \xmark        &51.2&55.3&65.6&11.9&32.8&41.1 \\   
                                                                                            & Track   & OWOD~\cite{joseph2021towards} &50.1&55.0&65.2&10.5&33.3&42.1      \\  
                                                                                            & Track   & Ours        &\textbf{53.5}&\textbf{55.9}&\textbf{66.3}&\textbf{14.1}&\textbf{33.5}&\textbf{42.6}   \\ \bottomrule  

                                                                                            
\end{tabular}
\caption{Performance of old and new classes in the ablation study on method components.  We ablate on the choice of pseudo-labels (PL) and contrastive (CT) loss for COOLer on Most$\rightarrow$Least setting on BDD100k. We compare training with our proposed  pseudo-labels generated by the tracker (Track) and the pseudo-labels by the detector (Det). We also compare our proposed class-incremental contrastive loss (Ours) with the contrastive loss proposed in OWOD~\cite{joseph2021towards}.}
\label{tab:ab_full}
\end{table*}

==> sup_tables/ab_oracle.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[htbp]
\centering
\footnotesize
\setlength\tabcolsep{2pt}
\renewcommand\arraystretch{0.9}
\begin{tabular}{@{}lcccccc@{}}
\toprule
   \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{Method:}\\\textbf{COOLer} 
   \end{tabular}}  & & \multicolumn{5}{c}{All Classes}                    \\ \cmidrule(l){3-7}                 &    Setting        & DetA & MOTA & HOTA & IDF1          & AssA          \\ \midrule
\multirow{4}{*}{\textbf{\bdd}}  
                        & Most$\rightarrow$Least                     & 27.9 & -2.6 & 34.4 & 42.6          & 43.8          \\  
                        & General$\rightarrow$Specific               & 32.4 & 28.6 & 38.5 & 48.2          & \textbf{47.0} \\  
                        & Vehicle$\rightarrow$Bike$\rightarrow$Human & 31.5 & 27.1 & 37.5 & 46.8          & 45.8 \\ \cmidrule(l){2-7}   & Oracle                         & 32.8 & 30.4 & 38.9 & 49.0          & 47.0                           \\ \midrule \midrule
\multirow{3}{*}{\textbf{\shift}}
                        & General$\rightarrow$Specific               & 44.2 & 46.0 & 50.8 & 57.0          & \textbf{59.5} \\  
                        & Vehicle$\rightarrow$Bike$\rightarrow$Human & 44.3 & 47.0 & 50.6 & \textbf{57.5} & \textbf{58.9}  \\  \cmidrule(l){2-7}   & Oracle                                     & 45.4 & 48.8 & 51.1 & 57.5          & 58.6          \\  \bottomrule
\end{tabular}
\caption{Comparison of COOLer and the oracle tracker.}
\label{tab:ab_oracle}
\end{table}

==> sup_tables/bdd_exp_full_overall.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[htbp]
\scriptsize 
\setlength\tabcolsep{1.6pt}
\renewcommand\arraystretch{0.9}

\end{table*}
% \tao{for this table and the next table: does it make sense to have the horizontal line disconnect between different ``xxx classes''? this could make the split of different classes more clear.}

==> sup_tables/dataset_statistics.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\setlength\tabcolsep{2pt}
\renewcommand\arraystretch{0.9}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
 Dataset              & Car     & Ped & Truck  & Bus   & Bike  & Rider & Motor & Train \\ \midrule
BDD100k        & 2098517 & 369798     & 149411 & 57860 & 25565 & 20107 & 12176 & 1620  \\
SHIFT & 677580  & 749640     & 145940 & 65367 & 52267 & -     & 74469 & -     \\ \bottomrule
\end{tabular}
\vspace{-2mm}
\caption{Class frequencies for BDD100k training split and the subset we used in SHIFT training split. }
\label{tab:statistics}
\end{table}

==> sup_tables/faster_ilod_plus.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[htbp]
\centering
\footnotesize
\setlength\tabcolsep{2pt}
\renewcommand\arraystretch{0.9}
\begin{tabular}{@{}lcccccc@{}}
\toprule
Setting (BDD100k)                                           & \multicolumn{1}{l}{Step} & DetA & MOTA & HOTA & IDF1 & AssA \\ \midrule
\multirow{4}{*}{Most$\rightarrow$Least}                     & 1                        & 49.0     & 46.4     &  51.7        &  63.0    &  \textbf{55.0}    \\
                                                            & 2                        & 42.2     &  27.3    & 47.8     &  57.3    &  \textbf{55.8}     \\
                                                            & 3                        & 36.1     &  -11.2    &   43.4   &  50.8    &  55.1     \\
                                                            & 4                        &  32.1    &  -19.4    &  40.1    & 47.1     & 52.6     \\ \midrule
General$\rightarrow$Specific                                & 1                        & 28.0     & -32.9     &  35.4    &  42.4    &  \textbf{47.9}    \\ \midrule
\multirow{2}{*}{Vehicle$\rightarrow$Bike$\rightarrow$Human} & 1                        &  27.0    &  -30.5    &  34.1    & 39.6     & \textbf{46.3}     \\
                                                            & 2                        &  28.7    &  14.8    &  35.8    & 43.9     &  \textbf{46.3}    \\ \bottomrule
\end{tabular}
\vspace{-2mm}
\caption{Performance of the modified Faster-ILOD on BDD100k. The results are average performance on all classes. The numbers that are better than COOLer are bolded.  }
\label{tab:faster_ilod_plus}
\end{table}

==> sup_tables/shift_exp_full_overall.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[htbp]
\scriptsize
\setlength\tabcolsep{1.6pt}
\renewcommand\arraystretch{0.9}

\end{table*}

==> sup_tables/shift_most_least.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[htbp]
\centering
\footnotesize
\setlength\tabcolsep{2pt}
\renewcommand\arraystretch{0.9}
\begin{tabular}{@{}lcccccc@{}}
\toprule
SHIFT Most$\rightarrow$Least                                              & Method      & DetA & MOTA & HOTA & IDF1 & AssA \\ \midrule
Step 0 (Pedestrian)                                                       & -           & 47.1 & 53.7 & 46.1 & 54.4 & 45.6 \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Step 1\\ + Car\end{tabular}}   & Fine-tuning &   25.2   & 25.8     & 28.5     &   30.9   & 32.8     \\
                                                                          & Det PL      &  47.9    & 44.6     &  46.8    & 49.7     &   47.8   \\
                                                                          & COOLer      & \textbf{48.1} & \textbf{50.9} & \textbf{50.9} & \textbf{57.0} & \textbf{55.1} \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Step 2\\ + Truck\end{tabular}} & Fine-tuning &  14.4    &  11.7    & 18.0     &  19.6    & 22.8     \\
                                                                          & Det PL      &  \textbf{46.0}    &  34.6    & 44.7     & 45.9     &  48.1    \\
                                                                          & COOLer      &  45.8    &  \textbf{45.2}    &  \textbf{51.5}    & \textbf{57.3}     &   \textbf{59.4}   \\ \bottomrule
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Step 3\\ + Motor\end{tabular}} & Fine-tuning &      &      &      &      &      \\
%                                                                           & Det PL      &      &      &      &      &      \\
%                                                                           & COOLer      &      &      &      &      &      \\ \bottomrule
\end{tabular}
\vspace{-2mm}
\caption{Results for Most$\rightarrow$Least Experiments on SHIFT. }
\label{tab:shift_most_least}
\end{table}
